PhysBrain: Human Egocentric Data as a Bridge from Vision Language Models to Physical Intelligence

Robotic generalization relies on physical intelligence: the ability to reason about state changes, contact-rich interactions, and long-horizon planning under egocentric perception and action. Vision Language Models (VLMs) are essential to Vision-Language-Action (VLA) systems, but the reliance on third-person training data creates a viewpoint gap for humanoid robots. Collecting massive robot-centric data is an ideal but impractical solution due to cost and diversity constraints. Conversely, human egocentric videos offer a highly scalable data source with rich interaction context, yet the embodiment mismatch prevents the direct application. To bridge this gap, we propose an Egocentric2Embodiment Translation Pipeline that transforms raw human egocentric videos into multi-level, schema-driven embodiment supervision with enforced evidence grounding and temporal consistency, enabling the construction of the Egocentric2Embodiment dataset (E2E-3M) at scale. An egocentric-aware embodied brain, termed PhysBrain, is obtained by training on the E2E-3M dataset. PhysBrain exhibits substantially improved egocentric understanding, particularly for planning. It provides an egocentric-aware initialization that enables more sample-efficient VLA fine-tuning and higher success rates, demonstrating effective transfer from human egocentric supervision to downstream robot control.

==> tab/app_dataset_tab.tex <==
% \begin{table*}[t]
% \centering
% \caption{\textbf{Taxonomy of Question Modes for Frame-Level Perception}. We deploy seven distinct query types to enforce a comprehensive understanding of the manipulation process, ranging from temporal sequencing to physical mechanics.} 
% \label{tab:vqa_modes} 
% \vskip 0.1in
% \resizebox{.99\textwidth}{!}{
%     \begin{tabular}{l|l|l}
%         \toprule
%         \textbf{Mode} & \textbf{Query Objective} & \textbf{Focus Point}\\
%         \midrule 
%         Summary & Synthesize the 1s clip into a concise overview & Abstract event summarization and key transitions \\
%         Temporal & Determine the chronological sequence of events & Flow of operations using explicit time connectives \\
%         Reasoning & Infer immediate outcomes or user intent & Causal relationships and goal deduction \\ 
%         Spatial & Analyze hand-object and object-surface relations & Geometric alignment, positioning, and adjustments \\ 
%         Mechanics & Describe execution details (grasp type, rotation) & Fine-grained action verbs and kinematic details \\
%         Trajectory & Track motion paths and endpoints & Directionality and movement termination \\
%         Attribute & Identify object states and visual properties & Physical characteristics relevant to interaction \\
%         \bottomrule 
%     \end{tabular}
% } 
% \vskip -0.1in
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{\textbf{Structured Annotation Schema for VLM Responses}. To prevent hallucination and ensure high fidelity, all generated answers must decompose the visual event into these five specific components.}
% \label{tab:annotation_schema}
% \vskip 0.1in
% \resizebox{\linewidth}{!}{%
%     \begin{tabular}{l|l|l}
%         \toprule
%         \textbf{Component} & \textbf{Example Content} & \textbf{Description} \\
%         \midrule
%         Subject Role & \texttt{Left hand}, \texttt{Right hand} & Explicit identification of the active manipulator \\
%         Contact Action & \texttt{grasps}, \texttt{stabilizes}, \texttt{releases} & Precise verbs describing the physical interaction \\
%         Object State & \texttt{broccoli held by stem}, \texttt{inserted} & The physical status of the object under manipulation \\
%         Temporal Connectives & \texttt{initially}, \texttt{then}, \texttt{meanwhile} & Structural words to enforce chronological coherence \\
%         Spatial Info & \texttt{into the center}, \texttt{above the pot} & Relative positioning and geometric context \\
%         \bottomrule
%     \end{tabular}%
% }
% \vskip -0.1in
% \end{table*}

==> tab/libero_tab.tex <==
\begin{table}[h]
  \centering
  \begin{adjustbox}{width=\linewidth}
  \begin{tabular}{l cc c c c c c}
    \toprule
    \textbf{Model} & \textbf{Steps} & \textbf{Epochs} & \textbf{Spatial} & \textbf{Object} & \textbf{Goal} & \textbf{Long} & \textbf{Avg} \\
    \midrule
    $\pi_0$+FAST~\cite{pertsch2025fast} & - & - & 96.4 & 96.8 & 88.6 & 60.2 & 85.5 \\
    OpenVLA-OFT~\cite{openvla-oft} & 175K & 223 & 97.6 & 98.4 & 97.9 & 94.5 & 97.1 \\
    $\pi_0$ & - & - & 96.8 & 98.8 & 95.8 & 85.2 & 94.1 \\
    GR00T-N1.5~\cite{bjorck2025gr00t} & 20K & 203  & 92.0 & 92.0 & 86.0 & 76.0 & 86.5 \\
    % GR00T-N1 (EO) & 20K $\times$ (8$\times$128) & 94.4 & 97.6 & 93.0 & 90.6 & 93.9 \\
    \midrule
    Qwen2.5-VL-FAST & 30K & 9.54 & 97.3 & 97.2 & 96.1 & 90.2 & 95.2 \\
    Qwen2.5-VL-OFT & 30K & 9.54  & 97.4 & 98.0 & 96.8 & 92.0 & 96.1 \\
    Qwen2.5-VL-GR00T & 30K & 9.54  & 97.8 & 98.2 & 94.6 & 90.8 & 95.4 \\
    \midrule
    Qwen3-vl-FAST & 30K & 9.54 & 97.3 & 97.4 & 96.3 & 90.6 & 95.4 \\
    Qwen3-vl-OFT & 30K & 9.54 & 97.8 & 98.6 & 96.2 & 93.8 & 96.6 \\
    Qwen3-vl-GR00T & 30K & 9.54 & 97.8 & 98.8 & 97.4 & 92.0 & 96.5 \\
    \midrule
    
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \vspace{0.3 em}
  \caption{Comparison of different VLA models on LIBERO. 
  We train one policy for all 4 suites. All scores are averaged over 500 trials for each task suite (10 tasks × 50 episodes). }
  \label{tab:vla_results}
\end{table}


==> tab/simplerenv_qwenpi_tab.tex <==
\definecolor{navyblue}{HTML}{0071BC}


\begin{table}[ht]
  \centering
  \caption{
    \textbf{Results of evaluating the VLA models with the WidowX robot in the SimplerEnv simulation environment}, where the VLM backbone is fine-tuned under the VLA paradigm following the \textbf{PhysPI architecture}.
    }
    \vspace{0.5em}
  \begin{adjustbox}{width=\linewidth}
  \begin{tabular}{l c c c c c}
    \toprule
    \textbf{Method}
     & \makecell[c]{\textbf{Put Spoon} \\ \textbf{on Towel}} 
     & \makecell[c]{\textbf{Put Carrot} \\ \textbf{on Plate}} 
     & \makecell[c]{\textbf{Stack Green Block} \\ \textbf{on Yellow Block}} 
     & \makecell[c]{\textbf{Put Eggplant} \\ \textbf{in Yellow Basket}} 
     & \textbf{Average} \\
    \midrule
    
    % --- VLM Baselines Header ---
    \rowcolor{navyblue!10}\multicolumn{6}{c}{\textit{\textbf{VLM Baselines}}} \\
    \addlinespace[0.2em]
    % ----------------------------

    Qwen2.5-VL-7B~\citep{Qwen25VL_2025_arXiv}       & 13.8  & 8.3   & 0.0   & 12.5  & 8.65 \\
    VST-RL-7B~\citep{VST_2025}                      & 29.2  & 20.9  & 4.2  & 89.6  & 35.9 \\
    Spatial-SSRL-7B~\cite{SpatialSSRL_2025}         & 19.4  & 16.7  & 2.1   & 90.3  & 32.1 \\
    
    \cmidrule(lr){1-6}  % 分割线

    \textbf{PhysBrain} (ours)  &  30.6 &  22.2 & 6.3 & 87.5 & \textbf{36.7}
    \\

    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \vspace{0.3 em}
  \label{tab:simplerenv_pi_results}
\end{table}
